Data-Efficient and Robust Trajectory Generation through Pathlet Dictionary Learning

Trajectory generation has recently drawn growing interest in privacy-preserving urban mobility studies and location-based service applications. Although many studies have used deep learning or generative AI methods to model trajectories and have achieved promising results, the robustness and interpretability of such models are largely unexplored. This limits the application of trajectory generation algorithms on noisy real-world data and their trustworthiness in downstream tasks. To address this issue, we exploit the regular structure in urban trajectories and propose a deep generative model based on the pathlet representation, which encode trajectories with binary vectors associated with a learned dictionary of trajectory segments. Specifically, we introduce a probabilistic graphical model to describe the trajectory generation process, which includes a Variational Autoencoder (VAE) component and a linear decoder component. During training, the model can simultaneously learn the latent embedding of pathlet representations and the pathlet dictionary that captures mobility patterns in the trajectory dataset. The conditional version of our model can also be used to generate customized trajectories based on temporal and spatial constraints. Our model can effectively learn data distribution even using noisy data, achieving relative improvements of $35.4\%$ and $26.3\%$ over strong baselines on two real-world trajectory datasets. Moreover, the generated trajectories can be conveniently utilized for multiple downstream tasks, including trajectory prediction and data denoising. Lastly, the framework design offers a significant efficiency advantage, saving $64.8\%$ of the time and $56.5\%$ of GPU memory compared to previous approaches.

==> method_revision_notes.tex <==
\section*{方法章节推导修改记录（Generative Model \& Variational Learning）}

本文件记录对方法章节中 \emph{Generative Model} 与 \emph{Variational learning} 两小节所做的数学与表述修改。每一条均包含「原文」「问题」「修改思路」「修改后结果（关键片段）」四个部分，便于日后回应审稿人或继续润色。

在下文中，符号约定与 \texttt{main.tex} 主文档保持一致。

\subsection*{1. 联合分布与 Markov 链写法不规范}

\paragraph{原文（节选）}
\begin{verbatim}
In this work, we formulate the compositional trajectory generation problem using 
the following Markov chain: z -> r -> x. ...
Since r is a binary vector, we model it as a Bernoulli distribution, 
r ~ Bernoulli(1 - p^n). The likelihood of the model P(x,z,r) can be factorized as
P(x,z,r) = P(x|r) P(r,z).
\end{verbatim}

\paragraph{问题}
\begin{itemize}
  \item 把联合分布 $P(\boldsymbol{x},\boldsymbol{z},\boldsymbol{r})$ 称为“likelihood of the model”在统计学上不规范；likelihood 一般指 $p(\boldsymbol{x}\mid\theta)$。
  \item 仅写成 $P(\boldsymbol{x}\mid\boldsymbol{r})P(\boldsymbol{r},\boldsymbol{z})$，未显式给出基于 Markov 链 $\boldsymbol{z}\to\boldsymbol{r}\to\boldsymbol{x}$ 的标准分解 $p(\boldsymbol{z})p(\boldsymbol{r}\mid\boldsymbol{z})p(\boldsymbol{x}\mid\boldsymbol{r})$，与图模型对应关系不够清晰。
\end{itemize}

\paragraph{修改思路}
\begin{itemize}
  \item 显式给出联合分布
  \[
    p(\boldsymbol{x},\boldsymbol{r},\boldsymbol{z})
    = p(\boldsymbol{x}\mid\boldsymbol{r};D)\,
      p_{\alpha}(\boldsymbol{r}\mid\boldsymbol{z})\,
      p(\boldsymbol{z}),
  \]
  并将其称为 joint distribution，而非 likelihood。
  \item 将 $p(\boldsymbol{z})$ 指定为高斯先验，$p_{\alpha}(\boldsymbol{r}\mid\boldsymbol{z})$ 与后续 Binary VAE 的生成分布保持一致。
\end{itemize}

\paragraph{修改后结果（关键片段）}
\begin{verbatim}
Under this construction, the joint distribution of all variables factorizes as
\begin{equation}
    p(\boldsymbol{x},\boldsymbol{r},\boldsymbol{z})
    = p(\boldsymbol{x}\mid\boldsymbol{r};D)\,
      p_{\alpha}(\boldsymbol{r}\mid\boldsymbol{z})\,
      p(\boldsymbol{z}),
\end{equation}
where p(\boldsymbol{z}) = N(0, I_K) and p_{\alpha}(\boldsymbol{r}\mid\boldsymbol{z})
is induced by the Bernoulli model above.
\end{verbatim}

\subsection*{2. $\boldsymbol{x}$ 既定义为二元向量又作为高斯变量使用}

\paragraph{原文（节选）}
\begin{verbatim}
... we assume random variable x in {0,1}^{|E|} is the observed trajectory ...
Specifically, the dependency between r and x ... follows a linear model
x = D r + eps, where eps ~ N(0, I).
\end{verbatim}

\paragraph{问题}
\begin{itemize}
  \item 从集合定义看，$\boldsymbol{x}\in\{0,1\}^{|E|}$ 是严格的二元向量；
  \item 但线性高斯模型 $\boldsymbol{x} = D\boldsymbol{r} + \boldsymbol{\epsilon}$ 意味着 $\boldsymbol{x}\mid\boldsymbol{r}\sim\mathcal{N}(D\boldsymbol{r}, I)$，这是连续观测模型；若不解释，会显得自相矛盾。
\end{itemize}

\paragraph{修改思路}
\begin{itemize}
  \item 保留 “$\{0,1\}^{|E|}$” 的离散表示以对应真实轨迹；
  \item 同时明确声明我们采用高斯观测模型作为连续化近似，并给出显式条件分布
  \[
    \boldsymbol{x}\mid\boldsymbol{r}\sim\mathcal{N}(D\boldsymbol{r}, \sigma^2 I_{|E|}).
  \]
\end{itemize}

\paragraph{修改后结果（关键片段）}
\begin{verbatim}
To enable gradient-based optimization, we adopt a continuous relaxation of the 
binary trajectory and assume a Gaussian observation model:
\begin{equation}
    \boldsymbol{z} \sim \mathcal{N}(\mathbf{0}, I_K), \qquad
    \boldsymbol{x} \mid \boldsymbol{r} \sim \mathcal{N}(D\boldsymbol{r}, \sigma^2 I_{|E|}),
\end{equation}
where D in {0,1}^{|E| x n} is the pathlet dictionary matrix and sigma^2 is a
fixed noise variance. Although \boldsymbol{x} is represented as a binary vector 
in {0,1}^{|E|}, the Gaussian observation model serves as a continuous 
approximation that facilitates differentiable training.
\end{verbatim}

\subsection*{3. $\boldsymbol{r}\sim Bernoulli(1-p^n)$ 维度错误且未体现对 $\boldsymbol{z}$ 的依赖}

\paragraph{原文（节选）}
\begin{verbatim}
Since r is a binary vector, we model it as a Bernoulli distribution,
r ~ Bernoulli(1 - p^n).
\end{verbatim}

\paragraph{问题}
\begin{itemize}
  \item $\boldsymbol{r}\in\{0,1\}^n$ 是向量，而 $Bernoulli(1-p^n)$ 是一维 Bernoulli，维度不匹配；
  \item 完全没有体现 $\boldsymbol{r}$ 对潜变量 $\boldsymbol{z}$ 的条件依赖，与 Markov 链 $\boldsymbol{z}\to\boldsymbol{r}$ 以及图中 $p_{\alpha}(\boldsymbol{r}\mid\boldsymbol{z})$ 不一致；
  \item 与后续 Binary VAE 中通过 $(\boldsymbol{m},\boldsymbol{p})$ 得到 $(1-\boldsymbol{p}^{\boldsymbol{m}})$ 的形式不统一。
\end{itemize}

\paragraph{修改思路}
\begin{itemize}
  \item 采用 Binary VAE 的分布形式：先由网络输出 $\boldsymbol{m}$ 和 $\boldsymbol{p}$，再对每一维 $r_j$ 定义
  \[
    r_j\mid\boldsymbol{z}\sim\mathrm{Bernoulli}\!\big(1-p_j^{m_j}\big),
    \quad j=1,\dots,n.
  \]
  \item 这样既保证维度正确，又显式依赖 $\boldsymbol{z}$，同时与重构项中的 $(1-\boldsymbol{p}^{\boldsymbol{m}})$ 精确对应。
\end{itemize}

\paragraph{修改后结果（关键片段）}
\begin{verbatim}
The dependency between \boldsymbol{z} and \boldsymbol{r} is modeled using a 
Binary VAE architecture. Given \boldsymbol{z}, two neural networks 
f_{alpha^m} and f_{alpha^p} produce the parameters \boldsymbol{m} and 
\boldsymbol{p}:
\begin{equation}
    \boldsymbol{m} = \exp\!\big(f_{\alpha^{m}}(\boldsymbol{z})\big), \qquad
    \boldsymbol{p} = \operatorname{sigmoid}\!\big(f_{\alpha^{p}}(\boldsymbol{z})\big),
\end{equation}
and each dimension of \boldsymbol{r} is generated as
\begin{equation}
    r_j \mid \boldsymbol{z} \sim \operatorname{Bernoulli}\!\big(1 - p_j^{m_j}\big),
    \quad j = 1,\dots,n.
\end{equation}
\end{verbatim}

\subsection*{4. “Variational learning of $P(\boldsymbol{r},\boldsymbol{z})$” 中变分对象与 ELBO 含义不清}

\paragraph{原文（节选）}
\begin{verbatim}
\subsection{Variational learning of P(r,z)}

The variational lower bound (ELBO) of Binary VAE model can be written as:
L_ELBO = E_{q(z|r)}[log p(r|z)] - KL[q(z|r) || p(z)].
\end{verbatim}

\paragraph{问题}
\begin{itemize}
  \item 小节标题写的是对 $P(\boldsymbol{r},\boldsymbol{z})$ 的变分学习，但 ELBO 实际是对 $\log p(\boldsymbol{r})$ 的下界；
  \item 文中没有给出
  \[
    \log p(\boldsymbol{r})
    = \log \int p_{\alpha}(\boldsymbol{r}\mid\boldsymbol{z})p(\boldsymbol{z})\,d\boldsymbol{z}
  \]
  以及“积分不可解 $\Rightarrow$ 需要变分近似”的推导逻辑。
\end{itemize}

\paragraph{修改思路}
\begin{itemize}
  \item 在小节开头显式写出目标：最大化 $\sum_i\log p(\boldsymbol{r}^{(i)})$，并给出对应积分形式；
  \item 说明使用 $q_{\phi}(\boldsymbol{z}\mid\boldsymbol{r})$ 近似后验 $p(\boldsymbol{z}\mid\boldsymbol{r})$，从而得到标准 ELBO 表达式。
\end{itemize}

\paragraph{修改后结果（关键片段）}
\begin{verbatim}
Given a collection of representation vectors, our goal is to learn the 
generative model p_alpha(r|z) p(z) by maximizing the marginal log-likelihood 
sum_i log p(r^{(i)}), where
\begin{equation}
    \log p(\boldsymbol{r}) = \log \int p_{\alpha}(\boldsymbol{r}\mid\boldsymbol{z})\,
    p(\boldsymbol{z})\,d\boldsymbol{z}.
\end{equation}
The integral over \boldsymbol{z} is intractable for a flexible neural decoder, 
so we resort to variational inference.
\end{verbatim}

\subsection*{5. 未明确定义编码器 $q_{\phi}(\boldsymbol{z}\mid\boldsymbol{r})$ 与训练目标}

\paragraph{原文（节选）}
\begin{verbatim}
Here, z is sampled from a normal distribution and used as the input to the 
neural network. The neural network outputs m and p as the parameters ...
The variational lower bound (ELBO) of Binary VAE model can be written as ...
\end{verbatim}

\paragraph{问题}
\begin{itemize}
  \item 文本只描述了 decoder（从 $\boldsymbol{z}$ 到 $\boldsymbol{r}$），但没有给出 encoder 的形式；
  \item 出现了 $q(\boldsymbol{z}\mid\boldsymbol{r})$，却没有说明其参数化方式。
\end{itemize}

\paragraph{修改思路}
\begin{itemize}
  \item 明确引入编码器网络 $g_{\phi}$，将 $q_{\phi}(\boldsymbol{z}\mid\boldsymbol{r})$ 写成对角高斯；
  \item 给出完整的 ELBO 表达式 $\mathcal{L}_{\text{ELBO}}(\boldsymbol{r})$，并将实际优化目标写成负 ELBO，即 $L_{\text{VAE}}$。
\end{itemize}

\paragraph{修改后结果（关键片段）}
\begin{verbatim}
We introduce an encoder network g_phi that parameterizes a variational posterior
\begin{equation}
    q_{\phi}(\boldsymbol{z}\mid\boldsymbol{r})
    = \mathcal{N}\big(\boldsymbol{\mu}_{\phi}(\boldsymbol{r}),
      \operatorname{diag}(\boldsymbol{\sigma}_{\phi}^2(\boldsymbol{r}))\big),
\end{equation}
and use the reparameterization trick to draw samples from 
q_{\phi}(\boldsymbol{z}\mid\boldsymbol{r}).

The evidence lower bound (ELBO) for log p(\boldsymbol{r}) is given by
\begin{equation}
    \mathcal{L}_{\text{ELBO}}(\boldsymbol{r})
    = \mathbb{E}_{q_{\phi}\left(\boldsymbol{z} \mid \boldsymbol{r}\right)}
        \left[\log p_{\alpha}\left(\boldsymbol{r} \mid \boldsymbol{z}\right)\right]
      - \operatorname{KL}\!\left[q_{\phi}\left(\boldsymbol{z} \mid \boldsymbol{r}\right) 
      \,\middle\|\, p\left(\boldsymbol{z}\right)\right],
\end{equation}
...
\begin{equation}
L_{\text{VAE}}
    = -\mathbb{E}_{q_{\phi}\left(\boldsymbol{z} \mid \boldsymbol{r}\right)}
        \left[\log p_{\alpha}\left(\boldsymbol{r} \mid \boldsymbol{z}\right)\right]
      + \operatorname{KL}\!\left[q_{\phi}\left(\boldsymbol{z} \mid \boldsymbol{r}\right) 
      \,\middle\|\, p\left(\boldsymbol{z}\right)\right].
\end{equation}
\end{verbatim}



